Learning-Augmented Sketches for Hessians

Sketching is a dimensionality reduction technique where one compresses a matrix by linear combinations that are chosen at random. A line of work has shown how to sketch the Hessian to speed up each iteration in a second order method, but such sketches usually depend only on the matrix at hand, and in a number of cases are even oblivious to the input matrix. One could instead hope to learn a distribution on sketching matrices that is optimized for the specific distribution of input matrices. We show how to design learned sketches for the Hessian in the context of second order methods. We prove that a smaller sketching dimension of the column space of a tall matrix is possible, given an oracle that can predict the indices of the rows of large leverage score. We design such an oracle for various datasets, and this leads to a faster convergence of the well-studied iterative Hessian sketch procedure, which applies to a wide range of problems in convex optimization. We show empirically that learned sketches, compared with their "non-learned" counterparts, do improve the approximation accuracy for important problems, including LASSO and matrix estimation with nuclear norm constraints.

==> embedding_oracle.tex <==
%!TeX root = main.tex
\section{Subspace Embedding with an Oracle}\label{sec:embedding_oracle}

First we prove the following lemma.

\begin{lemma}\label{lem:oracle_lemma}
Let $\delta\in (0,1/m)$. It holds with probability at least $1-\delta$ that
\[
\sup_{x\in\colspace(A)} \abs{\norm{Sx}_2^2 - \norm{x}_2^2} \leq \eps\norm{x}_2^2,
\]
provided that
\begin{gather*}
 m \gtrsim \eps^{-2}((d+\log m)\min\{\log^2(d/\eps),\log^2 m\} + d\log(1/\delta)), \\
 1 \gtrsim \eps^{-2}\nu((\log m)\min\{\log^2(d/\eps),\log^2 m\}+\log(1/\delta))\log(1/\delta).
\end{gather*}
\end{lemma}
\begin{proof}
We shall adapt the proof of Theorem 5 in~\cite{BDN15} to our setting. Let $T$ denote the unit sphere in $\colspace(A)$ and set the sparsity parameter $s=1$. Observe that $\norm{Sx}_2^2 = \norm{x_I}_2^2 + \norm{Sx_{I^c}}_2^2$, and so it suffices to show that
\[
\Pr\left\{ \abs{\norm{S'x_{I^c}}_2^2 - \norm{x_{I^c}}_2^2} > \eps \right\} \leq \delta
\]
for $x\in T$. We make the following definition, as in (2.6) of~\cite{BDN15}: 
\[
A_{\delta,x} := \sum_{i=1}^m \sum_{j\in I^c} \delta_{ij}x_j e_i\otimes e_{j},
\]
and thus, $S'x_{I^c} = A_{\delta,x}\sigma$. Also by $\E\norm{S'x_{I^c}}_2^2 = \norm{x_{I^c}}_2^2$, one has
\begin{equation}\label{eqn:oracle_basic}
\sup_{x\in T}\abs{\norm{S'x_{I^c}}_2^2 - \norm{x_{I^c}}_2^2} = \sup_{x\in T} \abs{ \norm{A_{\delta,x}\sigma}_2^2 - \E \norm{A_{\delta,x}\sigma}_2^2  }.
\end{equation}
Now, in (2.7) of~\cite{BDN15} we instead define a seminorm
\[
\norm{x}_\delta = \max_{1\leq i\leq m}\left(\sum_{j\in I^c} \delta_{ij} x_j^2\right)^{1/2}.
\]
Then (2.8) continues to hold, and (2.9) as well as (2.10) continue to hold if the supremum in the left-hand side is replaced with the left-hand side of~\eqref{eqn:oracle_basic}. At the beginning of Theorem 5, we define $U^{(i)}$ to be $U$, but each row $j\in I^c$ is multiplied by $\delta_{ij}$ and each row $j\in I$ is zeroed out. Then we have in the first step of (4.5) that 
\[
\sum_{j\in I^c} \delta_{ij} \abs{\sum_{k=1}^d g_k\langle f_k, e_j\rangle}^2 \leq \norm{U^{(i)}g}_2^2, 
\]
instead of equality. One can verify that the rest of (4.5) goes through. It remains true that $\norm{\cdot}_\delta \leq (1/\sqrt{s})\norm{\cdot}_2$, and thus (4.6) holds. One can verify that the rest of the proof of Theorem 5 in~\cite{BDN15} continues to hold if we replace $\sum_{j=1}^n$ with $\sum_{j\in I^c}$ and $\max_{1\leq j\leq n}$ with $\max_{j\in I^c}$, noting that
\[
\E\sum_{j\in I^c}\delta_{ij}\norm{P_E e_j}_2^2 = \frac{s}{m}\sum_{j\in I^c}\langle P_E e_j,e_j\rangle \leq \frac{s}{m}d
\]
and
\[
\E (U^{(i)})^\ast U^{(i)} = \sum_{j\in I^c}(\E\delta_{ij}) u_j u_j^\ast \preceq \frac{1}{m}.
\]
Thus, the symmetrization inequalities on 
\[
\norm{\sum_{j\in I^c} \delta_{ij}\norm{P_E e_j}_2^2}_{L_\delta^p} \quad\text{and}\quad \norm{\sum_{j\in I^c}\delta_{ij}u_j u_j^\ast}_{L_\delta^p}
\]
continue to hold. The result then follows, observing that $\max_{j\in I^c} \norm{P_E e_j}^2\leq \nu$.
\end{proof}

The subspace embedding guarantee now follows as a corollary.
\begin{theorem}
Let $\nu = \eps/d$. Suppose that
$m = O((d/\eps^2)(\polylog(1/\eps) + \log(1/\delta)))$, $\delta = O(\eps^2/(d\polylog(d/\eps)))$ and $d = \Omega((1/\eps)\polylog(1/\eps)\log^2(1/\delta)) $. Then, there exists a distribution on $S$ with $m + |I|$ rows such that 
\[
\Pr\left\{ \forall x\in\colspace(A), \abs{\norm{Sx}_2^2 - \norm{x}_2^2} > \eps\norm{x}_2^2 \right\} \leq \delta.
\]
\end{theorem}
\begin{proof}
One can verify that the two conditions in  Lemma~\ref{lem:oracle_lemma} are satisfied if
\begin{gather*}
\delta \leq \frac{1}{m}, \\
m \gtrsim \frac{d}{\eps^2}\left(\polylog(\frac{d}{\eps})+\log\frac{1}{\delta}\right), \\
d \gtrsim \frac{1}{\eps}\left(\log\frac{1}{\delta}\right)\left(\polylog(\frac{d}{\eps})+\log\frac{1}{\delta}\right).
\end{gather*}
The last condition is satisfied if
\[
d \gtrsim \frac{1}{\eps}\left(\log^2 \frac{1}{\delta}\right)\polylog\left(\frac{1}{\eps}\right).
\]
The first condition is satisfied if
\[
\delta \leq \frac{\eps^2}{d\polylog(\frac{d}{\eps})}. \qedhere
\]
\end{proof}

\subsection{Experiments}

In this section, we give the empirical results for the above learning-based subspace embedding, where we use the GHG dataset and the following synthetic dataset:
\begin{itemize}
\item \textbf{Synthetic Data}: We generate pairs $(A_i, B_i)$ as $B_i = A_i X_i^{*} + W_i$, where $A_i \in \R^{n \times d}$,  $X_i^{*} \in \R^{d}$,  and $W_i \in \R^{d}$ is noise with i.i.d.\ $N(0, \sigma^2)$ entries. Here we set $n = 1000, d = 10$, and $|(A_i,B_i)| = 100$. We set $r = d / \eps$ leverage scores of $A_i$ to be large and the remaining ones to be small. We generate $A_i$ as follows: we pick a random matrix $C \in \R^{r \times d}$ with orthonormal columns and sample a matrix $D \in \R^{(n - r) \times d}$ with i.i.d. $N(0, \tau^2)$ entries, where $\tau$ is sufficiently small. Then we perform the Gram-Schmidt orthogonalization for the columns of $(\begin{smallmatrix} C \\ D\end{smallmatrix})$ and set $U$ to be the resulting matrix. Finally we pick a random orthogonal matrix $V \in \R^{d \times d}$ and a positive diagonal matrix $\Sigma$  and let $A = U \Sigma V^\top$. Here, we set $n = 1000, d = 10$, $|(A_i,B_i)| = 100$, $\epsilon = 0.1$, $0.2$, $\sigma = 0.1$, and $\tau = r / 10 n$.
\end{itemize}	

\paragraph{Experimental Setting} We consider the least squares task on the above two datasets and compare the performance of random \textsc{Count-Sketch} matrices with and without oracle access, where we assume that the oracle can, upon querying a row index $i$, return whether row $i$ of $A$ has a large leverage score. Given the sketch matrix $S$, we define the error of $S$ over the dataset $A$ to be $\mathcal{L}(S, A) = \frac{1}{N}\sum_{i=1}^N \mathcal{L}(S,A_i)$ where $\mathcal{L}(S,A_i) = \normtwo{A_i((SA_i)^{+}SB) - B_i}$.

\begin{table}[h]
	\centering  
	\caption{Average error for least squares regression}  
	\label{table:1}  
	
	\begin{tabular}{|c|c|c|c|}  
		\hline  
		& & & \\[-6pt]  
		& $m = 5d$ & $m = 7d$ & $m = 10d$ \\  
		\hline
		& & & \\[-6pt]  
		Synthetic($\eps = 0.1$, without oracle) & 0.318 & 0.230& 0.161\\
		\hline
		
		& & & \\[-6pt]  
		Synthetic($\eps = 0.1$, with oracle) &0.161&  0.088& 0.039 \\
		\hline
		& & & \\[-6pt]  
		Synthetic($\eps = 0.2$, without oracle) & 0.321 & 0.221& 0.160\\
		\hline
		& & & \\[-6pt]  
		Synthetic($\eps = 0.2$, with oracle) &  0.238& 0.167& 0.086\\
		\hline
		& & & \\[-6pt]  
		GHG (without oracle) & 5.02 & 3.36& 2.29\\
		\hline
		& & & \\[-6pt]  
		GHG (with oracle) & 3.46 & 2.13& 1.25\\
		\hline
	\end{tabular}
	
\end{table}

A comparison of results is given in Table~\ref{table:1}, where we take an average over $10$ independent trials. For each experiment, we assume oracle access which returns whether a row $i$ belongs to the top $m/5$ rows of largest leverage scores.


==> experiment.tex <==
%!TeX root = main.tex
\section{IHS Experiments}\label{sec:ihs_exp}

\textbf{Training.} We learn the sketching matrix in each iteration (also called a round) separately. Recall that in the $(t+1)$-st round of IHS, the optimization problem we need to solve~\eqref{eqn:IHS update} depends on $x_t$. An issue is that we do not know $x_t$, which is needed to generate the training data for the $(t + 1)$-st round. Our solution is to use the sketch matrix in the previous round to obtain $x_t$ by solving~\eqref{eqn:IHS update}, and then use it to generate the training data in the next round. 
That is, in the first round, we train the sketch matrix $S_1$ to solve the problem
$
x_{1} = \argmin_{x \in \mathcal{C}} \frac{1}{2} \normtwo{S_1 Ax}^2 - \inner{A^\top b , x}
$
and use $x_1$ to generate the training data for the optimization problem for $x_2$, and so on. The loss function we use is the unsketched objective function in the $(t+1)$-st iteration, i.e., $\mathcal{L}(S_{t+1},A) = \frac{1}{2}\norm{A(x_{t+1}-x_t)}_2^2 - \langle A^T(b-Ax_t),x_{t+1}-x_t\rangle$, where $x_{t+1}$ is the solution to~\eqref{eqn:IHS update} and thus depends on $S_{t+1}$.

\textbf{Comparison.} We compare the learned sketch against three classical sketches: Gaussian, \textsc{Count-Sketch}, and SJLT (see Section~\ref{sec:prelim}) in all experiments. The quantity we compare is a certain error, defined individually for each problem, in each round of the iteration of the IHS or as a function of the runtime of the algorithm. All of our experiments are conducted on a laptop with a 1.90GHz CPU and 16GB RAM.

\begin{figure}[tb]
\begin{minipage}{0.47\textwidth}
    \centering
    \includegraphics[width=0.87\textwidth]{co_new.png}
    \caption{Test error of LASSO on CO emission dataset, $m=3d$}\label{fig:lasso_CO_2}
\end{minipage}
\hfill
\begin{minipage}{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{co.png}
    \caption{Test error of LASSO on CO emissions dataset, $m=5d$}\label{fig:lasso_CO}
\end{minipage}
\end{figure}

\begin{figure}[H]
\begin{minipage}{0.47\textwidth}
    \centering
    \includegraphics[width=0.87\textwidth]{ghg_new.png}
    \caption{Test error of LASSO on GHG dataset, $m=3.5d$}\label{fig:lasso_greenhouse_2}
\end{minipage}
\hfill
\begin{minipage}{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{ghg.png}
    \caption{Test error of LASSO on greenhouse gas dataset, $m=6d$}\label{fig:lasso_greenhouse}
\end{minipage}
\end{figure}

\subsection{LASSO}

We define an instance of LASSO regression as
\begin{equation}\label{eqn:LASSO}
x^* = \argmin_{x \in \R^d} \frac{1}{2} \normtwo{Ax - b}^2 + \lambda \normone{x}, 
\end{equation}
where $\lambda$ is a parameter. We use two real-world datasets:
\begin{itemize}
    \item \textbf{CO emission}\footnote{\url{https://archive.ics.uci.edu/ml/datasets/Gas+Turbine+CO+and+NOx+Emission+Data+Set}}: the dataset contains 9 sensor measures aggregated over one hour (by means of average or sum), which can help to predict the CO emission. We divide the raw data into $120$ ($A_i$, $b_i$) such that $A_i \in \R^{300 \times 9}$, $b_i \in \R^{300 \times 1}$. The data in each matrix is sorted in chronological order. $|(A, b)_{\train}| =
96$, $|(A, b)_{\test}| = 24$.
    
    \item \textbf{Greenhouse gas} (GHG)\footnote{\url{https://archive.ics.uci.edu/ml/datasets/Greenhouse+Gas+Observing+Network}}: time series of measured greenhouse gas concentrations in the California atmosphere. Each $(A, b)$ corresponds to a different measurement location. $A_i \in \R^{327 \times 14}$, $b_i \in \R^{327 \times 1}$, and $|(A, b)_{\train}| =
400$, $|(A, b)_{\test}| = 100$. (This dataset was also used in \cite{LLVWW20}.)
\end{itemize}

We set $\lambda=1$ in the LASSO regression~\eqref{eqn:LASSO}. We choose $m=3d,5d$ for the CO emission dataset and $m=3.5d,6d$ for the GHG dataset. We consider the error $(\frac{1}{2}\norm{Ax-b}_2^2+\norm{x}_1)-(\frac12\norm{Ax^\ast-b}_2^2+\norm{x^\ast}_1)$ and take an average over five independent trials. We plot in (natural) logarithmic scale the mean errors of the two datasets in Figures~\ref{fig:lasso_CO_2} to~\ref{fig:lasso_greenhouse}. 
We can observe that the learned sketches consistently outperform the classical random sketches in all cases. Note that our sketch size is much smaller than the theoretical bound. For a smaller sketch size, classical random sketches converge slowly or do not yield stable results, while the learned sketches can converge to a small error quickly. For larger sketch sizes, all three classical sketches have approximately the same order of error, and the learned sketches reduce the error by a $5/6$ to $7/8$ factor in all iterations.


\subsection{Matrix Estimation with Nuclear Norm Constraint} 
\label{sec:nuclear_exp}
In many applications, for the problem
\[
X^*:= \argmin_{X \in \R^{d_1 \times d_2}} \fnorm{AX - B}^2 \;,  
\]
it is reasonable to model the matrix $X^*$ as having low rank. Similar to $\ell_1$-minimization for compressive sensing, a standard relaxation of the rank constraint is to minimize the nuclear norm of $X$, defined as $\norm{X}_{\ast} := \sum_{j = 1}^{\min\{d_1, d_2\}} \sigma_j(X)$, where $\sigma_j(X)$ is the $j$-th largest singular value of $X$.

Hence, the matrix estimation problem we consider here is
 \[
 X^*:= \argmin_{X \in \R^{d_1 \times d_2}} \fnorm{AX - B}^2  \text{  such that } \norm{X}_{\ast} \le \rho,
 \]
where $\rho > 0$ is a user-defined radius as a regularization parameter.

We conduct experiments on the following two datasets:

\begin{itemize}
    \item \textbf{Synthetic Dataset}: We generate the pair $(A_i, B_i)$ as $B_i = A_i X_i^{*} + W_i$, where $A_i \in \R^{n \times d_1}$ with i.i.d $N(0, 1)$ entries. $X_i^{*} \in \R^{d_1 \times d_2}$ is a matrix with rank at most $r$. $W_i$ is noise with i.i.d.\ $N(0, \sigma^2)$ entries. Here we set $n = 500, d_1 = d_2 = 7, r = 3, \rho = 30$. $|(A,B)|_{\train} = 270$, $|(A, B)|_{\test} = 30$.
    \item \textbf{Tunnel}\footnote{{\url{https://archive.ics.uci.edu/ml/datasets/Gas+sensor+array+exposed+to+turbulent+gas+mixtures}}}: The data set is a time series of gas concentrations measured by eight sensors in a wind tunnel. Each $(A, B)$ corresponds to a different data collection trial. $A_i \in \R^{13530 \times 5}, B_i \in \R^{13530 \times 6}$,
    $|(A,B)|_{\train} = 144$, $|(A, B)|_{\test} = 36$. The same dataset and parameters were also used by \cite{LLVWW20} for regression tasks. In our nuclear norm constraint, we set $\rho = 10$. 
\end{itemize}

We choose $m=40, 50$ for the synthetic dataset and $m = 10, 50$ for the Tunnel dataset and define the error to be $\frac{1}{2}(\fnorm{AX - B}^2 - \fnorm{AX^* - B}^2)$. For each data point, we take the average error of five independent trials. The mean errors of the two datasets when $m = 50$ are plotted in a (natural) logarithmic scale in Figures~\ref{fig:matrix_est_synthetic} and~\ref{fig:matrix_est_tunnel}. We observe that the classical sketches yield approximately the same order of error, while the learned sketches improve the error by at least 30\% for the synthetic dataset and surprisingly by at least 95\% for the Tunnel dataset. The huge improvement on the Tunnel dataset may be due to the fact that the matrices $A_i$ have many duplicate rows. We also plot the results when $m = 10$ or $40$ in Figures~\ref{fig:matrix_est_synthetic_new} and~\ref{fig:matrix_est_tunnel_new}, which show that the learned sketches yield much smaller errors than the random sketches and the random sketches could converge significantly more slowly with considerably larger errors in the first several rounds.

\begin{figure}[tb]
\begin{minipage}{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth,clip,trim = {0 0 0 20px}]{gau.png}
    \caption{Test error of matrix estimation on synthetic data, $m=50$}\label{fig:matrix_est_synthetic}
\end{minipage}
\hfill
\begin{minipage}{0.47\textwidth}
    \centering
    \includegraphics[width=0.87\textwidth,clip,trim = {0 0 0 20px}]{gau_new.png}
    \caption{Test error of matrix estimation on synthetic dataset, $m=40$}\label{fig:matrix_est_synthetic_new}
\end{minipage}
\end{figure}

\begin{figure}[tb]
\centering
\begin{minipage}{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth,clip,trim = {0 0 0 20px}]{gas.png}
    \caption{Test error of matrix estimation on Tunnel dataset, $m=50$}\label{fig:matrix_est_tunnel}
\end{minipage}
\hfill
\begin{minipage}{0.47\textwidth}
    \centering
    \includegraphics[width=0.87\textwidth,clip,trim = {0 0 0 20px}]{gas_new.png}
    \caption{Test error of matrix estimation on Tunnel dataset, $m=10$}\label{fig:matrix_est_tunnel_new}
\end{minipage}
\end{figure}

\subsection{Runtime of Learned Sketches}

As stated in Section~\ref{sec:prelim}, our learned sketch matrices $S$ are all \textsc{Count-Sketch}-type matrices (each column contains a single nonzero entry), the matrix product $SA$ can thus be computed in $O(\nnz(A))$ time and the overall algorithm is expected to be fast. To verify this, we plot an error-versus-runtime plot for matrix estimation with nuclear norm constraint tasks in Figure~\ref{fig:gas_time} (corresponding to the datasets in Figure~\ref{fig:matrix_est_tunnel}). The runtime consists only of the time for sketching and solving the optimization problem and does not include the time for loading the data. We run the same experiment three times. Each time we take an average over all test data. From the plot we can observe that the learned sketch and \textsc{Count-Sketch} have the fastest runtimes, which are slightly faster than that of the SJLT and significantly faster than that of the Gaussian sketch.


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth,clip,trim = {0 0 0 10px}]{gas_time.png}
    \caption{Test error of matrix estimation on Tunnel dataset}\label{fig:gas_time}
\end{figure}

==> experiment2.tex <==
%!TeX root = main.tex
\section{Fast Regression Experiment}

We consider the unconstrained least-squares problem, i.e.,~\eqref{eqn:LASSO} with $\lambda=0$, using the CO emission %, greenhouse gas datasets, 
and the following Census dataset:

\begin{itemize}
	\item \textbf{Census data}\footnote{{\url{https://github.com/chocjy/randomized-quantile-regression-solvers/tree/master/matlab/data}}}: this dataset consists of annual salary and related features on people who reported
that they worked 40 or more weeks in the previous year and worked 35 or more hours per week. We randomly sample $5000$ instances to create $(A_i, b_i)$, where $A \in \R^{5000 \times 11}$ and $b \in \R^{5000 \times 1}$, $|(A,B)|_{\train} = 160$, $|(A, B)|_{\test} = 40$.
\end{itemize}




\paragraph{Training.} We optimize the learned sketch $S_1$ by gradient descent (Algorithm~\ref{alg:train_hessian_regression}), where $\mathcal{L}(S,A) = \kappa(A R_1^{-1})$, where $R_1$ is computed as in Algorithm~\ref{alg:fast_regression} and $\kappa(M)$ denotes the condition number of a matrix $M$. 

Next we discuss how to generate the training data. We use Newton's method to solve an unconstrained convex optimization problem, in the $t$-th round, we need to solve a regression problem $\min_z \norm{A^\top A z - y}_2$ (see~\eqref{eqn:newton_update}), where $A = \nabla^2 f(x_t)^{1/2}$ and $y = \nabla f(x_t)$, both depend on the previous solution $x_t$. Hence, we take $x_t$ to be the solution obtained from Algorithm~\ref{alg:fast_regression} using the learned sketch $S_t$, and this generates $A$ and $y$ for the $(t+1)$-st round.

\paragraph{Experiment.} For the CO emission dataset, we set $m = 70$, and for the Census dataset, $m=500$.
For the $\eta$ in the Algorithm~\ref{alg:fast_regression}, we set $\eta = 1$ for the first round and $\eta = 0.2$ for the subsequent rounds for the CO emission dataset, and $\eta = 1$ in all rounds for the Census dataset. 

We examine the accuracy of the subproblem~\eqref{eqn:hessian_minimization} and define the error to be $\normtwo{A^\top A Rz_t - y} / \normtwo{y}$. We run the first three subroutines of solving the subproblem for both CO emission and Census datasets. 
The average error of three independent trials is plotted in Figures~\ref{fig:fr_co} and \ref{fig:fr_census}. We observe that for the CO emission dataset, the classical sketches have a similar performance and the learned sketches lead to a fast convergence in the subroutine with the first-round error at least 80\% smaller; 
for the Census dataset, the learned sketch achieves the smallest error in all three rounds, where we reduce about $60\%$ error in the first round and about $50\%$ error in the third round. Note that the learned sketch always considerably outperforms \textsc{Count-Sketch} in all cases.


\begin{figure}[t]
\centering
%\begin{minipage}{0.33\textwidth}
    \includegraphics[clip,trim={20px 0 25px 30px},width=0.32\textwidth]{fr_co1.png}
%\end{minipage}
%
%\begin{minipage}{0.33\textwidth}
    \includegraphics[clip,trim={20px 0 25px 30px},width=0.32\textwidth]{fr_co2.png}
%\end{minipage}
%
%\begin{minipage}{0.33\textwidth}
    \includegraphics[clip,trim={20px 0 25px 30px},width=0.32\textwidth]{fr_co3.png}
%\end{minipage}
    \caption{Test error of fast regression for the CO emission dataset, first three calls in solving an unconstrained least-squares}\label{fig:fr_co}
\end{figure}

\begin{figure}[t]
\centering
%\begin{minipage}{0.33\textwidth}
    \includegraphics[clip,trim={20px 0 25px 30px},width=0.325\textwidth]{cen1.png}
%\end{minipage}
%\begin{minipage}{0.33\textwidth}
    \includegraphics[clip,trim={20px 0 25px 30px},width=0.32\textwidth]{cen2.png}
%\end{minipage}
%\begin{minipage}{0.33\textwidth}
    \includegraphics[clip,trim={20px 0 25px 30px},width=0.32\textwidth]{cen3.png}
%\end{minipage}
    \caption{Test error of fast regression for the Census dataset, first three calls in solving an unconstrained least-squares}\label{fig:fr_census}
\end{figure}

%\end{minipage}

%\end{wrapfigure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.7\textwidth,height=0.25\textwidth]{fr2.png}
%    
%\end{figure}


==> greenhouse_exp.tex <==
%!TeX root = main.tex
% \section{IHS Experiment: LASSO}\label{sec:lasso_appendix}

% \begin{figure}[H]
% \begin{minipage}{0.47\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{co.png}
%     \caption{Test error of LASSO on CO emissions dataset, $m=5d$}\label{fig:lasso_CO}
% \end{minipage}
% \hfill
% \begin{minipage}{0.47\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{ghg.png}
%     \caption{Test error of LASSO on greenhouse gas dataset, $m=6d$}\label{fig:lasso_greenhouse}
% \end{minipage}
% \end{figure}


% \section{IHS Experiment: Support Vector Machines}\label{sec:svm_appendix}

% We plot in a (natural) logarithmic scale the mean errors of the three datasets in Figures~\ref{fig:gaussian} to \ref{fig:number}.

% \begin{figure}[H]
% \centering
% \begin{minipage}{0.325\textwidth}
%     \includegraphics[width=\textwidth]{gaussian.png}
%     \caption{Test error of SVM on random Gaussian dataset}\label{fig:gaussian}
% \end{minipage}
% \hfill
% \begin{minipage}{0.325\textwidth}
%     \includegraphics[width=\textwidth]{flocking.png}
%     \caption{Test error of SVM on swarm behavior dataset}\label{fig:flocking}
% \end{minipage}
% \hfill
% \begin{minipage}{0.325\textwidth}
%     \includegraphics[width=\textwidth]{number.png}
%     \caption{Test error of SVM on Gisette dataset}\label{fig:number}
% \end{minipage}
% \end{figure}

% \section{IHS Experiment: Matrix Estimation with a Nuclear Norm Constraint}\label{sec:exp_nuclear}

% As stated in Section~\ref{sec:nuclear_exp}, the mean errors of the two datasets when $m = 40$ for the synthetic dataset and $m = 10$ for the Tunnel dataset are plotted in a (natural) logarithmic scale in Figures~\ref{fig:matrix_est_synthetic_new} and~\ref{fig:matrix_est_tunnel_new}.

% \begin{figure}[h]
% \centering
% \begin{minipage}{0.47\textwidth}
% 	\centering
%     \includegraphics[width=\textwidth]{gau_new.png}
% %    \vspace{-0.3cm}
%     \caption{Test error of matrix estimation on synthetic dataset, $m=40$}\label{fig:matrix_est_synthetic_new}
% \end{minipage}
% \hfill
% \begin{minipage}{0.47\textwidth}
% 	\centering
%     \includegraphics[width=\textwidth]{gas_new.png}
% %    \vspace{-0.6cm}
%     \caption{Test error of matrix estimation on Tunnel dataset, $m=10$}\label{fig:matrix_est_tunnel_new}
% \end{minipage}
% \end{figure}

%
%\section{Fast Regression Experiment: Greenhouse Gas}\label{sec:greenhouse_gas_exp}
%
%We set $m = 100$, $\eta=0.2$ in the first round and $\eta=1$ in the second round. The mean errors of the first two calls of the fast regression subroutine are plotted in Figure~\ref{fig:fr_ghg}. We can observe that Gaussian and sparse JL sketches have a significantly better performance than \textsc{Count-Sketch}, and the learned sketch shows again a significant reduction of more than 50\% in the first-round error.
%
%\begin{figure}[h]
%\begin{minipage}{0.45\textwidth}
%    \centering
%    \includegraphics[clip,trim={20px 0 25px 30px},width=0.8\textwidth]{fr_ghg1.png}
%\end{minipage}
%\hfill
%\begin{minipage}{0.45\textwidth}
%	\centering
%    \includegraphics[clip,trim={20px 0 25px 20px},width=0.8\textwidth]{fr_ghg2.png}
%\end{minipage}
%\caption{Test error of fast regression for the greenhouse gas emission dataset, first two calls in solving an unconstrained least-squares}\label{fig:fr_ghg}
%\end{figure}


==> leverage_score_exp.tex <==
\section{Leverage Score Experiment}

In this section, we give the empirical results for learning-based subspace embedding, where we use the GHG dataset and the following synthetic dataset:
\begin{itemize}[leftmargin=20pt]
\item \textbf{Synthetic Data}: We generate pairs $(A_i, B_i)$ as $B_i = A_i X_i^{*} + W_i$, where $A_i \in \R^{n \times d}$,  $X_i^{*} \in \R^{d}$,  and $W_i \in \R^{d}$ is noise with i.i.d.\ $N(0, \sigma^2)$ entries. Here we set $n = 1000, d = 10$, and $|(A_i,B_i)| = 100$. We set $r = d / \eps$ leverage scores of $A_i$ to be large and the remaining ones to be small. We generate $A_i$ as follows: we pick a random matrix $C \in \R^{r \times d}$ with orthonormal columns and sample a matrix $D \in \R^{(n - r) \times d}$ with i.i.d. $N(0, \tau^2)$ entries, where $\tau$ is sufficiently small. Then we perform the Gram-Schmidt orthogonalization for the columns of $(\begin{smallmatrix} C \\ D\end{smallmatrix})$ and set $U$ to be the resulting matrix. Finally we pick a random orthogonal matrix $V \in \R^{d \times d}$ and a positive diagonal matrix $\Sigma$  and let $A = U \Sigma V^\top$. Here, we set $n = 1000, d = 10$, $|(A_i,B_i)| = 100$, $\epsilon = 0.1$, $0.2$, $\sigma = 0.1$, and $\tau = r / 10 n$.
\end{itemize}	

\paragraph{Experimental Setting} We consider the least squares task on the above two datasets and compare the performance of random \textsc{Count-Sketch} matrices with and without oracle access, where we assume that the oracle can, upon querying a row index $i$, return whether row $i$ of $A$ has a large leverage score. Given the sketch matrix $S$, we define the error of $S$ over the dataset $A$ to be $\mathcal{L}(S, A) = \frac{1}{N}\sum_{i=1}^N \mathcal{L}(S,A_i)$ where $\mathcal{L}(S,A_i) = \normtwo{A_i((SA_i)^{+}SB) - B_i}$.

\begin{table}[h]
	\centering  
	\caption{Average error for least squares regression}  
	\label{table:1}  
	
	\begin{tabular}{|c|c|c|c|}  
		\hline  
		& & & \\[-6pt]  
		& $m = 5d$ & $m = 7d$ & $m = 10d$ \\  
		\hline
		& & & \\[-6pt]  
		Synthetic($\eps = 0.1$, without oracle) & 0.318 & 0.230& 0.161\\
		\hline
		
		& & & \\[-6pt]  
		Synthetic($\eps = 0.1$, with oracle) &0.161&  0.088& 0.039 \\
		\hline
		& & & \\[-6pt]  
		Synthetic($\eps = 0.2$, without oracle) & 0.321 & 0.221& 0.160\\
		\hline
		& & & \\[-6pt]  
		Synthetic($\eps = 0.2$, with oracle) &  0.238& 0.167& 0.086\\
		\hline
		& & & \\[-6pt]  
		GHG (without oracle) & 5.02 & 3.36& 2.29\\
		\hline
		& & & \\[-6pt]  
		GHG (with oracle) & 3.46 & 2.13& 1.25\\
		\hline
	\end{tabular}
	
\end{table}

A comparison of results is given in Table~\ref{table:1}, where we take an average over $10$ independent trials. For each experiment, we assume oracle access which returns whether a row $i$ belongs to the top $m/5$ rows of largest leverage scores.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

